On the Weihrauch degree of the additive Ramsey theorem

We characterize the strength, in terms of Weihrauch degrees, of certain problems related to Ramsey-like theorems concerning colourings of the rationals and of the natural numbers. The theorems we are chiefly interested in assert the existence of almost-homogeneous sets for colourings of pairs of rationals respectively natural numbers satisfying properties determined by some additional algebraic structure on the set of colours. In the context of reverse mathematics, most of the principles we study are equivalent to $\Sigma^0_2$-induction over $\mathrm{RCA}_0$. The associated problems in the Weihrauch lattice are related to $\mathrm{TC}_\mathbb{N}^*$, $(\mathrm{LPO}')^*$ or their product, depending on their precise formalizations.

==> macrosQ.tex <==
\usepackage{cite}
%\usepackage[top=3cm, bottom=2cm, left=3cm, right=3cm]{geometry}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[super]{nth}
%\usepackage[english]{babel}
\usepackage{array}
\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{hyperref}
\hypersetup{hidelinks}
\usepackage{url}
\usepackage{stmaryrd}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{todonotes}
\usepackage{mathbbol}
\usepackage{mathtools}
%\usepackage{amsthm}
\usepackage{bm,accents}
\usepackage{appendix}
\usepackage{xfrac}
\usepackage{relsize}
\usepackage{faktor}
\usepackage{xspace}
\usepackage[all]{xy}
\usepackage[shortcuts]{extdash}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}[theorem]{Remark}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{question}[theorem]{Question}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{numclaim}[theorem]{Claim}
\newtheorem{subclaim}[theorem]{Subclaim}
%\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{hypothesis}[theorem]{Hypothesis}

\newenvironment{notations}[1][Notations]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\ident}[2]{\newcommand{#1}{\ensuremath{\texorpdfstring{\mathrm{#2}}{#2}}\xspace}}
\newcommand{\operator}[2]{\newcommand{#1}{\ensuremath{\texorpdfstring{\mathop{#2}\xspace}{#2}}}}

\newcommand{\fun}[3]{\ensuremath{#1\colon #2 \to #3}}
\newcommand{\funmap}[3]{\ensuremath{#1\colon #2 \mapsto #3}}
\newcommand{\parfun}[3]{\ensuremath{#1\colon #2 \rightharpoonup #3}}

\ident{\dom}{dom}
\ident{\rg}{rg}
\ident{\id}{id}
\ident{\sgn}{sgn}

\newcommand{\Image}{\text{Im}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\inl}{{\sf inl}}
\newcommand{\inr}{{\sf inr}}
\newcommand{\bnfalt}{\mathrel{|}}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\bbN}{\mathbb N}
\newcommand{\bbtwo}{\mathbb{2}}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbC}{\mathbb C}
\newcommand{\cO}{\mathcal O}
\newcommand{\cF}{\mathcal F}
\newcommand{\bigslant}[2]{{\left.\raisebox{.2em}{$#1$}\middle/\raisebox{-.2em}{$#2$}\right.}}
\newcommand{\append}{\raisebox{.2em}{$\frown$}}
%\newcommand{\nil}{\langle \rangle}
\newcommand{\nil}{\epsilon}
\newcommand{\op}{\text{op}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\powersetinh}[1]{\mathcal{P}_*(#1)}
\newcommand{\powersetfin}{\mathcal{P}_{\ident{fin}}}
\newcommand{\eqdef}{\mathrel{\mathop{:}=}}
\newcommand{\cc}{\aleph_0\mathfrak{C}}
\newcommand{\chains}{\mathfrak{C}}
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}
\newcommand{\lex}{\ident{lex}}
\newcommand{\len}{\ident{len}}
\newcommand{\SW}{{\sf SW}} %scattered words
\newcommand{\CW}[1]{{#1}^\circ} %countable words
\newcommand{\leaves}{\cL}
\newcommand{\nodes}{\cN}
\newcommand{\children}{\cC}
\newcommand{\symdiff}{\triangle}
\newcommand{\compat}{\mathrel{\top}}
\newcommand{\tuple}[1]{( #1 )}
\newcommand{\ftuple}[1]{\langle #1 \rangle}
\newcommand{\card}[1]{{| #1 |}}
\newcommand{\setlt}{<_1}
\newcommand{\setle}{\le_1}
\newcommand{\partto}{\rightharpoonup}
\newcommand{\midca}{\mathrel{|}}

\newcommand{\GrJ}{\mathrel{\mathcal{J}}}
\newcommand{\GrH}{\mathrel{\mathcal{H}}}
\newcommand{\GrL}{\mathrel{\mathcal{L}}}
\newcommand{\GrR}{\mathrel{\mathcal{R}}}
%\newcommand{\dom}{\text{dom}}
\newcommand{\lang}{\cL}

\newcommand{\oointerval}[2]{{]#1,#2[}}
\newcommand{\cointerval}[2]{{[#1,#2[}}
\newcommand{\ccinterval}[2]{{[#1,#2]}}
\newcommand{\rtvalfm}{{\sf RT_{\ident{val}}}}
\newcommand{\rtsetfm}{{\sf RT_{\ident{set}}}}

\newcommand{\comment}[1]{}

%  Leszek's stuff + reverse math stuff
\newcommand{\ca}{\textrm{-}\mathsf{CA}_0}
\newcommand{\ind}{\textrm{-}\mathsf{IND}}
\newcommand{\aca}{\mathsf{ACA}_0}
\newcommand{\atr}{\mathsf{ATR}_0}
\newcommand{\rca}{\mathsf{RCA}_0}
\newcommand{\wkl}{\mathsf{WKL}_0}
\newcommand{\rt}{\mathsf{RT}}
\newcommand{\srt}{\mathsf{SRT}}
\newcommand{\mso}{\mathsf{MSO}}
\newcommand{\abr}{\mathsf{ABR}_0}
\newcommand{\bca}{\textrm{-}\mathsf{BCA}_0}

\newcommand{\michal}[1]{\todo[inline,backgroundcolor=red!25]{{\bf MS}: #1}}
\newcommand{\pierre}[1]{\todo[inline,backgroundcolor=blue!25]{{\bf PP}: #1}}
\newcommand{\leszek}[1]{\todo[inline,backgroundcolor=green!25]{{\bf LK}: #1}}

\newcommand{\revom}{{\omega^\op}}
\newcommand{\omegaalg}{\tau}
\newcommand{\revomalg}{{\tau^\op}}
\newcommand{\etaalg}{\kappa}

\newcommand{\cv}{\ident{conv}}
\newcommand{\st}{\ident{scat}}
\newcommand{\sh}{\ident{shuf}}
\newcommand{\ddi}{d.d.i.}

\newcommand{sztindtext}{$\Sigma^0_2$-induction}
\newcommand{sztind}{$\Sigma^0_2\ind$}

\theoremstyle{plain}
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
\def\rep@title{#2 \ref{##1}}%
\begin{rep@theorem}}%
{\end{rep@theorem}}}

\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}
\newreptheorem{proposition}{Proposition}
\newreptheorem{conjecture}{Conjecture}
\newreptheorem{claim}{Claim}

